Developing Optimization-Based Inverter Models for Short Circuit Studies

As inverter-based generation becomes more common in distribution networks, it is important to create models for use in optimization-based problems that accurately represent their non-linear behavior when saturated. This work presents models for grid-following and grid-forming inverters, and demonstrates their use in optimization-based fault studies. The developed models are shown to provide results in line with experimental tests from literature; however, grid-forming inverter models fail to provide feasible solutions for certain fault types even when currents, voltages, and powers from the models seem reasonable. This work lays down the foundation for the development of relaxed models for both grid-following and grid-forming inverter models for use in optimization problems.

==> comments.tex <==

DUE 4/30/23
Authors should consider revising their paper, based on the following comments:
1. Please clarify the novelty of the study.
- we need to hit the point that the focus is on building models that will eventually be converted to linear convex approximates. ALREADY STATED IN THE INTRODUCTION SO I'D SAY THIS IS ALREADY DONE!
[Yes, that the inverter models are setup for an optimization problem... ] Agree
2. Provide the main assumptions pertaining to Eqs. (1)-(10).
- this is confusing they are the basic power flow equations defined in constraints, maybe say that? 
- there are a few assumptions: harmonic voltages/currents can be neglected, generators capability curves can be approximated by a box. I don't think that It's needed for the system to be kron-reduced for this formulation, maybe check with David/Juan?
[Yes, Newton-Raphson, coordinates, etc formulation of pf equations (what is the format of the equations, we have a few options), and then second, yes there are some assumptions, frequency close to nominal, load models assumptions, are they constant power, ZIP, etc... ]
- I think that while explicitly stating the assumptions, it's also important to state that these are standard assumptions for an unbalanced powerflow and cite something like OpenDSS, CymDist, Gridlab-D, Kersting's book, etc.
3. Improve the discussion of results. 
[There are quite a few images, connect them a bit more with the text] 
4. Improve the conclusion: the main findings resulting from the study should be clearly identified. Suggested improvements and future direction of this work could also be included.
[A combination of all of the above, recap of all the new discussion added ...]- 
Emphasize how this is leading to convex/linear models for inverters under fault studies
5. Improve the figures, some are not legible. DONE
6. Improve the title of the paper. DONE
- Development of Inverter Models for Optimization-based Shor t Circuit Studies.
- Approximate Methods for Modeling Inverter in Optimization-based Short Circuit Studies
- Approximate Methods for Modeling Short-Circuit Currents from Inverter
- [Developing Optimization-Based Inverter Models for Short Circuit Studies]

The current ($I_a$)  DONE
The current [$A$] DONE
